Series2Graph: Graph-based Subsequence Anomaly Detection for Time Series

Subsequence anomaly detection in long sequences is an important problem with applications in a wide range of domains. However, the approaches proposed so far in the literature have severe limitations: they either require prior domain knowledge used to design the anomaly discovery algorithms, or become cumbersome and expensive to use in situations with recurrent anomalies of the same type. In this work, we address these problems, and propose an unsupervised method suitable for domain agnostic subsequence anomaly detection. Our method, Series2Graph, is based on a graph representation of a novel low-dimensionality embedding of subsequences. Series2Graph needs neither labeled instances (like supervised techniques) nor anomaly-free data (like zero-positive learning techniques), and identifies anomalies of varying lengths. The experimental results, on the largest set of synthetic and real datasets used to date, demonstrate that the proposed approach correctly identifies single and recurrent anomalies without any prior knowledge of their characteristics, outperforming by a large margin several competing approaches in accuracy, while being up to orders of magnitude faster. This paper has appeared in VLDB 2020.

==> Challenges.tex <==
\section{Why is Finding Anomalies Challenging?}
\label{sec:challenges}

Nm can be equivalent to $m_th$ discord ...
the problem is with false positive and brute force over large m ... (already present fix!)
presence of anomalies, with different semantics ( Top-K discords problem, multiple normal model needed, discords is )
 

%\commentRed{I add here, what Paul added at the beginning}

%\subsection{Why Finding Anomalies is challenging?}
%Outliers (a.k.a anomalies) can be subjective to the analyzed domain. They might be rare events patterns in the entire signal, or repeated one at the same time.  But how can we define the word rare. According to the matrix profile method,a metadata that give us a significant information about the recurrence of some patterns, an anomaly is defined as a discord, i.e a pattern with the worst match in the entire series. However, could an anomaly be also a recurrent pattern? 
Anomaly discovery might be sensitive to the analyzed domain. In certain systems, an anomalous behavior can be identified as a rare and deviated pattern. This problem has been extensively studied in \cite{DBLP:conf/edbt/Senin0WOGBCF15,Keogh2007,Liu2009,DBLP:conf/adma/FuLKL06,DBLP:conf/icdm/YehZUBDDSMK16,DBLP:conf/sdm/BuLFKPM07}, where fast and scalable \discord discovery techniques are proposed.
On the contrary, when a system is subject to the presence of many abnormal patterns, searching the $m^{th}$ discords, where $m$ is unknown, turns out to be prohibitively expensive, in terms of time and memory, especially when $m$ is large. %and might be sensitive to false positive, as we shown in the introduction. 
Nevertheless, we might still want to apply a $m^{th}$ discords discovery technique, such as the one introduced by Yankov et al.\footnote{The authors of this paper, define the problem as $k^{th}$ discord discovery.}~\cite{DBLP:conf/icdm/YankovKR07}, which considers the highest $m^{th}$ nearest neighbor distance of each subsequence, in order to find groups of repeated and similar anomalies pattern.
We see at least two drawbacks in this technique. First, we need to know $m$ a priori, and second, if we select a large $m$ iterating until \textit{1}, will allow to potentially discover all the outliers clusters, but incurring also into false positive. 
In Figure~\ref{falsePositiveDiscord}.a), we report a bunch of point subsequences in a bi-dimensional space, where a group of outliers (red/dark) is present. Clearly, if we set $m=3$, the sequence $A$, is discovered as $3^{rd} discord$ (highest distance to the $3^{rd}$ nearest neighbor). We also note that, if $m$ is set to \textit{11}, the sequence $B$, is erroneously detected as discord, since visually it does not belong to any outliers cluster. 
  
\begin{figure}[tb]
 	\centering
 	\includegraphics[trim={1cm 15cm 19.5cm 3cm}, scale=0.9]{images/falsePositiveDiscord}
 	\caption{Sequences in a bi-dimensional space. In red, the outliers cluster. (a) A and B are respectively the $3^{rd}$ and $11^{th}$ discords. (b) The anomalies are detected as the farthest points to $N_{M}$, which is the barycenter point of the cluster (draw in green).}
 	\label{falsePositiveDiscord}
\end{figure}
  
  
  
  
%\begin{figure}[tb]
%	\centering
%	\includegraphics[trim={0cm 14.5cm 5cm 2.5cm}, scale=0.70]{../images/SingleAnomaly.pdf}
%	\caption{(a) MBA ECG recording (\textit{2500} points snippet from patient 803), with annotated ventricular premature contraction (V). (b) Matrix profile of the snippet, reporting the Euclidean distances of the best non trivial matches.}
%	\label{singleAnomaly}
%\end{figure}
%
%%In the figure \ref{recurrentAnom}, according to the annotation of the Physiobank dataset, the pattern indicated by the red triangle are Premature ventricular contraction. These patterns have a different shape than the regular beats, but unfortunately happen more than once. In this case, the matrix profile will have some difficulties to differentiate the normal beat from the anomalies, because both of these two patterns happen more than once in the whole series. Without any notion of truth, the anomalies could be considered as normal behavior. The figure \ref{selfjoinExample} outlines the inefficiency of the matrix profile for series with recurrent anomalies.
%In order to justify our statement, we show a real example, coming from the health-care domain. In Figure~\ref{singleAnomaly}.(a) we report a snippet of the MIT-BIH Arrhythmia Database (MBA) ECG recording \cite{Goldbergere215,Moody}, where we can find expert-annotated anomalies such as \textit{Premature ventricular contraction} (V) and \textit{Superventricular premature beats} (S), which are highly repeated along the whole \textit{half hour} recording, sampled at 360\textit{Hz}. Here we arbitrarily selected a part containing exactly one single anomaly (V).  
%Our goal is to our new and more abstract definition of anomalies taking into account a notion of truth, and the possible high frequency of appearance by merging the significant information that the matrix profile can give to us.
%This definition need to be able to differentiate all the following cases of outliers.

%\noindent{\bf Single  \anomaly}

%In Figure~\ref{singleAnomaly}.(b) we plot the matrix profile \cite{DBLP:conf/icdm/YehZUBDDSMK16} of the signal in (a), which is a meta-data series reporting for each subsequence of a given length, the Euclidean distance to its nearest neighbor in the signal itself, excluding the trivial matches. Note that, in the matrix profile the Euclidean distances are found at the offset of the corresponding subsequences. Those distances are generally coupled with their positions, we omit here this information. The state-of-the-art \discord discovery works computing the matrix profile, which contains the $Top-k-1^{st}$ discords ranking distances. In our case, the real \anomaly, whose position is contoured by the highest peak in (b), is the $Top-1-1^{st}$ discord.             

%\begin{figure}[tb]
%	\centering
%	\includegraphics[scale=0.25]{../images/visuWrongDetection.jpg}
%	\caption{Matrixe profile of the ECG of the patient 803 from PhysioBank. The red rectangle represent the anomalies supposed to be discord but considered as a motif by the matrix profile}
%	\label{selfjoinExample}
%\end{figure}

%\begin{figure}[tb]
%	\centering
%	\includegraphics[trim={0cm 14.5cm 5cm 2.5cm}, scale=0.70]{../images/MultiAnomaly.pdf}%\subsection{Two Similar Outliers}
%	\caption{(a) MBA ECG recording (\textit{5000} points snippet from patient 803), with four annotated ventricular premature contraction (V). (b) Matrix profile of the snippet, reporting the Euclidean distances of the best non trivial matches.}%
%	\label{recurrentAnom}
%\end{figure}	

%\noindent{\bf Multiple \anomaly} 

%However, in Figure~\ref{recurrentAnom}.(a) we have shown a slightly larger part (\textit{5000} pts.) of the same MBA signal, which contains many (V) and (S). We note that the anomalies are very similar and the computed matrix profile in Figure~\ref{recurrentAnom}.(b), clearly does not provide any cues, since the anomalous subsequences are not distinguishable from any normal heartbeats, solely looking at the matrix profile. This represents a limitation of this technique. 
%%Given also the fact that, the current state-of-the-art techniques, suitable for $Top-k-1^{st}$ discovery permit to scale up to small $k$ \cite{DBLP:conf/sdm/BuLFKPM07,DBLP:conf/edbt/Senin0WOGBCF15,Parameter-Free_Discord}, if we are interested in considering the whole MBA dataset, containing thousands of anomalous subsequences, this latter would not represent a viable solution.
We are thus in the need for a new method, which takes into account the variety of (highly) repeated anomalies ($Top-rec-k$ anomalies).

%As a matter of fact, finding anomalies is challenging in the definition of what we are looking for. Where the previous technique have difficulties to find {\bf multiple anomalies of same type}, we will try to overpass this problem, and go even further by detecting {\bf multiple anomalies of different type}, without for instance taking into consideration the $V$ and $S$ anomalies separately.

%In the case when we have a single abnormal pattern that correspond to a pair of two patterns with the largest distance with it nearest neighbours, the existing techniques perform very well to find the pattern that correspond to our definition of anomalies. Indeed, matrix profile leads to a straightforward and efficient solution for the discord problem. In the figure \ref{SingleDiscord}, the first plot is a time series from human motion recognition ~\cite{Paper_koegh_Themis}. The second one is the plot of the corresponding matrix profile. We can indeed see that the matrix profile technique successfully found the anomaly.
%
%
%\begin{figure}[tb]
%	\centering
%	\includegraphics[scale=0.25]{../images/singleDiscord.png}
%	\caption{In this case, the cardinality of the abnormals patterns is one. Therefore our definition of anomalies correspond to the discord definition}
%	\label{SingleDiscord}
%\end{figure}
%
%
%\subsection{Multiple Outliers of the Same Type}
%
%Now let consider that an outlier happens several time in the time series, which is very probable in a very long one. In other words, more than one similar outliers. In that case, it will not be consider as a Discord anymore, but as a motifs. The figure \ref{selfjoinExample} shows indeed that previous technique are not able to detect them as anomalies.
%
%
%
%\subsection{Multiple Outliers of Different Types}
%
%Finally, let consider the case when there is more than one outliers in a series that are not similar to one another. Previous approaches would need different algos to identify them all {\bf ??? references? ???}. Indeed, discord-based approaches would need to find the discord, remove it from the sequence, find the next one, etc, leading to slow performances.

%{\bf ??? references? ???}

%{\bf ??? is this true? can eh discord algos find all the discords in 1 pass? ???} {\bf ??? example, time experiment ???}


